Computably Continuous Reinforcement-Learning Objectives are PAC-learnable

In reinforcement learning, the classic objectives of maximizing discounted and finite-horizon cumulative rewards are PAC-learnable: There are algorithms that learn a near-optimal policy with high probability using a finite amount of samples and computation. In recent years, researchers have introduced objectives and corresponding reinforcement-learning algorithms beyond the classic cumulative rewards, such as objectives specified as linear temporal logic formulas. However, questions about the PAC-learnability of these new objectives have remained open. This work demonstrates the PAC-learnability of general reinforcement-learning objectives through sufficient conditions for PAC-learnability in two analysis settings. In particular, for the analysis that considers only sample complexity, we prove that if an objective given as an oracle is uniformly continuous, then it is PAC-learnable. Further, for the analysis that considers computational complexity, we prove that if an objective is computable, then it is PAC-learnable. In other words, if a procedure computes successive approximations of the objective's value, then the objective is PAC-learnable. We give three applications of our condition on objectives from the literature with previously unknown PAC-learnability and prove that these objectives are PAC-learnable. Overall, our result helps verify existing objectives' PAC-learnability. Also, as some studied objectives that are not uniformly continuous have been shown to be not PAC-learnable, our results could guide the design of new PAC-learnable objectives.

==> aaai23-aux.tex <==
\begin{filecontents}
{aaai23.aux}
\relax 
\bibstyle{aaai23}
\citation{smcbltl,dorsa14,gltl17,hasanbeig2019reinforcement,omegaregularrl19,rewardmachine1,ltlf-rl,osbert,bozkurt2020control,rdp21}
\citation{rewardmachine1}
\citation{bozkurt2020control}
\citation{ltlnonpac22}
\citation{pacmdpsmcconfidenceinterval,smcbltl,ufukpacmdpltl14,rdp21}
\citation{alur2021framework}
\citation{dorsa14,gltl17,hasanbeig2019reinforcement,omegaregularrl19,rewardmachine1,osbert,bozkurt2020control}
\citation{bazille20}
\citation{rewardmachine1,bozkurt2020control,gltl17}
\newlabel{seq-notation}{{2}{2}}
\newlabel{seq-notation@cref}{{[footnote][2][]2}{[1][2][]2}}
\citation{rewardmachine1}
\citation{rewardmachine1}
\newlabel{sec:reward_machine_example}{{3}{3}}
\newlabel{sec:reward_machine_example@cref}{{[section][3][]3}{[1][3][]3}}
\citation{tlhierarchy}
\providecommand*\caption@xref[2]{\@setref\relax\@undefined{#1}}
\newlabel{fig:reward-machine}{{1}{4}}
\newlabel{fig:reward-machine@cref}{{[figure][1][]1}{[1][4][]4}}
\newlabel{sec:uniform_continuity_implies_pac}{{4}{4}}
\newlabel{sec:uniform_continuity_implies_pac@cref}{{[section][4][]4}{[1][4][]4}}
\newlabel{sec:continuity-implies-pac-learnability}{{4.2}{4}}
\newlabel{sec:continuity-implies-pac-learnability@cref}{{[subsection][2][4]4.2}{[1][4][]4}}
\newlabel{thm:environment-specific-pac-learnable-iff-uniform-continuous}{{1}{4}}
\newlabel{thm:environment-specific-pac-learnable-iff-uniform-continuous@cref}{{[theorem][1][]1}{[1][4][]4}}
\citation{ipoc19}
\citation{ipoc19}
\citation{weihrauch2000computable}
\citation{weihrauch2000computable}
\citation{weihrauch2000computable}
\citation{weihrauch2000computable}
\citation{gltl17}
\newlabel{thm:environment-generic-pac-learnable-if-uniform-continuous}{{2}{5}}
\newlabel{thm:environment-generic-pac-learnable-if-uniform-continuous@cref}{{[corollary][2][]2}{[1][5][]5}}
\newlabel{lemma:label_preserves_uniform_continuity}{{3}{5}}
\newlabel{lemma:label_preserves_uniform_continuity@cref}{{[lemma][3][]3}{[1][5][]5}}
\newlabel{sec:computability}{{4.3}{5}}
\newlabel{sec:computability@cref}{{[subsection][3][4]4.3}{[1][5][]5}}
\newlabel{def:computable-objective}{{7}{5}}
\newlabel{def:computable-objective@cref}{{[definition][7][]7}{[1][5][]5}}
\newlabel{thm:computable-implies-uc}{{4}{5}}
\newlabel{thm:computable-implies-uc@cref}{{[theorem][4][]4}{[1][5][]5}}
\newlabel{thm:objective-pac-learnable-if-computable}{{5}{5}}
\newlabel{thm:objective-pac-learnable-if-computable@cref}{{[theorem][5][]5}{[1][5][]5}}
\citation{tlhierarchy}
\citation{hasanbeig2019reinforcement,omegaregularrl19,bozkurt2020control}
\citation{bozkurt2020control}
\citation{dorsa14,hasanbeig2019reinforcement,omegaregularrl19}
\citation{bozkurt2020control}
\citation{bozkurt2020control}
\citation{Sickert2016LimitDeterministicBA}
\citation{bozkurt2020control}
\citation{bozkurt2020control}
\newlabel{sec:theorem-apps}{{5}{6}}
\newlabel{sec:theorem-apps@cref}{{[section][5][]5}{[1][5][]6}}
\newlabel{lst:simple-reward-machine-objective-impl}{{1}{6}}
\newlabel{lst:simple-reward-machine-objective-impl@cref}{{[listing][1][]1}{[1][6][]6}}
\newlabel{sec:ltl-in-the-limit-spec-intro}{{5.2}{6}}
\newlabel{sec:ltl-in-the-limit-spec-intro@cref}{{[subsection][2][5]5.2}{[1][6][]6}}
\citation{bozkurt2020control}
\citation{dorsa14,hasanbeig2019reinforcement,omegaregularrl19}
\citation{bozkurt2020control}
\citation{bozkurt2020control}
\citation{bozkurt2020control}
\citation{bozkurt2020control}
\citation{bozkurt2020control}
\citation{rewardmachine1}
\citation{stochasticrewardmachine22}
\citation{dorsa14,omegaregularrl19,hasanbeig2019reinforcement}
\citation{smcbltl,osbert,ltlf-rl}
\bibdata{paper}
\bibcite{alur2021framework}{{1}{2021}{{Alur et~al.}}{{Alur, Bansal, Bastani, and Jothimurugan}}}
\newlabel{eq:bozkurt_objective_def}{{1}{7}}
\newlabel{eq:bozkurt_objective_def@cref}{{[equation][1][]1}{[1][6][]7}}
\newlabel{lst:ldba-objective-impl}{{2}{7}}
\newlabel{lst:ldba-objective-impl@cref}{{[listing][2][]2}{[1][7][]7}}
\bibcite{pacmdpsmcconfidenceinterval}{{2}{2019}{{Ashok, K{\v {r}}et{\'i}nsk{\'y}, and Weininger}}{{}}}
\bibcite{bazille20}{{3}{2020}{{Bazille et~al.}}{{Bazille, Genest, Jegourel, and Sun}}}
\bibcite{bozkurt2020control}{{4}{2020}{{Bozkurt et~al.}}{{Bozkurt, Wang, Zavlanos, and Pajic}}}
\bibcite{rewardmachine1}{{5}{2019}{{Camacho et~al.}}{{Camacho, Toro~Icarte, Klassen, Valenzano, and McIlraith}}}
\bibcite{stochasticrewardmachine22}{{6}{2022}{{Corazza, Gavran, and Neider}}{{}}}
\bibcite{ipoc19}{{7}{2019}{{Dann et~al.}}{{Dann, Li, Wei, and Brunskill}}}
\bibcite{ufukpacmdpltl14}{{8}{2014}{{Fu and Topcu}}{{}}}
\bibcite{ltlf-rl}{{9}{2019}{{Giacomo et~al.}}{{Giacomo, Iocchi, Favorito, and Patrizi}}}
\bibcite{omegaregularrl19}{{10}{2019}{{Hahn et~al.}}{{Hahn, Perez, Schewe, Somenzi, Trivedi, and Wojtczak}}}
\bibcite{hasanbeig2019reinforcement}{{11}{2019}{{Hasanbeig et~al.}}{{Hasanbeig, Kantaros, Abate, Kroening, Pappas, and Lee}}}
\bibcite{smcbltl}{{12}{2012}{{Henriques et~al.}}{{Henriques, Martins, Zuliani, Platzer, and Clarke}}}
\bibcite{osbert}{{13}{2019}{{Jothimurugan, Alur, and Bastani}}{{}}}
\bibcite{gltl17}{{14}{2017}{{Littman et~al.}}{{Littman, Topcu, Fu, Isbell, Wen, and MacGlashan}}}
\bibcite{tlhierarchy}{{15}{1987}{{Manna and Pnueli}}{{}}}
\bibcite{rdp21}{{16}{2021}{{Ronca and De~Giacomo}}{{}}}
\bibcite{dorsa14}{{17}{2014}{{Sadigh et~al.}}{{Sadigh, Kim, Coogan, Sastry, and Seshia}}}
\bibcite{Sickert2016LimitDeterministicBA}{{18}{2016}{{Sickert et~al.}}{{Sickert, Esparza, Jaax, and Křet{\'i}nsk{\'y}}}}
\bibcite{weihrauch2000computable}{{19}{2000}{{Weihrauch}}{{}}}
\bibcite{ltlnonpac22}{{20}{2022}{{Yang, Littman, and Carbin}}{{}}}
\gdef \@abspage@last{8}
\end{filecontents}
